Neural Ray-Tracing: Learning Surfaces and Reflectance for Relighting and View Synthesis

Recent neural rendering methods have demonstrated accurate view interpolation by predicting volumetric density and color with a neural network. Although such volumetric representations can be supervised on static and dynamic scenes, existing methods implicitly bake the complete scene light transport into a single neural network for a given scene, including surface modeling, bidirectional scattering distribution functions, and indirect lighting effects. In contrast to traditional rendering pipelines, this prohibits changing surface reflectance, illumination, or composing other objects in the scene. In this work, we explicitly model the light transport between scene surfaces and we rely on traditional integration schemes and the rendering equation to reconstruct a scene. The proposed method allows BSDF recovery with unknown light conditions and classic light transports such as pathtracing. By learning decomposed transport with surface representations established in conventional rendering methods, the method naturally facilitates editing shape, reflectance, lighting and scene composition. The method outperforms NeRV for relighting under known lighting conditions, and produces realistic reconstructions for relit and edited scenes. We validate the proposed approach for scene editing, relighting and reflectance estimation learned from synthetic and captured views on a subset of NeRV's datasets.

==> discussion.tex <==
\section{Discussion}
Our explicit modelling of analytic and learned components allows us to directly model light
transport, and allows for efficient surface intersections, permitting approximations of
soft-shadows, accurate surface reconstruction and fast higher-order light computations. Due to
the prohibitive cost and noise introduced through soft-shadows introduced by NeRV, we explore
an alternative to soft-shadows using an occlusion predicting MLP, and find it to be effective.

Comparing to prior work on view-synthesis and scene reconstruction, our work matches the
performance of existing methods, while providing stronger physical interpretation thanks to our
decomposed scene representations, and physically accurate reconstruction. Exploring even more
compact and easily-trainable decomposed scene representations is a direction we leave to be
explored in future work.

\section{Limitations}
While our methodology is efficient at accurate reconstruction of surfaces, it fails in certain
cases. For example, when the model has transparency, such as water, it would have difficulty
modelling transmittance through the medium. Another case of decreased performance is if there is
significant specularity, as the diffuse model may be unable to accurately capture the average
value. In such a case, it may be suitable to use a more robust analytic BRDF, such as a
Cook-Torrance microfacet BRDF. A computational burden may also be the random sampling as opposed
to importance sampling, and finding an effective solution for modelling the integral of the
learned BSDF could lead to better sampling and thus more efficient pathtracing.


